Intrinsic limits to gene regulation by global crosstalk

Gene regulation relies on the specificity of transcription factor (TF) - DNA interactions. In equilibrium, limited specificity may lead to crosstalk: a regulatory state in which a gene is either incorrectly activated due to noncognate TF-DNA interactions or remains erroneously inactive. We present a tractable biophysical model of global crosstalk, where many genes are simultaneously regulated by many TFs. We show that in the simplest regulatory scenario, a lower bound on crosstalk severity can be analytically derived solely from the number of (co)regulated genes and a suitable parameter that describes binding site similarity. Estimates show that crosstalk could present a significant challenge for organisms with low-specificity TFs, such as metazoans, unless they use appropriate regulation schemes. Strong cooperativity substantially decreases crosstalk, while joint regulation by activators and repressors, surprisingly, does not; moreover, certain microscopic details about promoter architecture emerge as globally important determinants of crosstalk strength. Our results suggest that crosstalk imposes a new type of global constraint on the functioning and evolution of regulatory networks, which is qualitatively distinct from the known constraints acting at the level of individual gene regulatory elements.

==> combreg_table.tex <==
\begin{table}
\label{Tab:combreg}
\begin{tabular}[b]{|c|c|c|>{\centering}m{1cm}|>{\centering}m{1cm}|>{\centering}m{1cm}|>{\centering}m{1cm}|c|c|}
\hline 
 &  &  & \multicolumn{4}{c|}{crosstalk if gene needs to be} &  & \tabularnewline
 & configuration & activity & \multirow{2}{1cm}{ON} & \multicolumn{3}{c|}{OFF, C can be} & Energy & Weight\tabularnewline
\cline{5-7} 
 & (XY) &  &  & X & Y & none &  & \tabularnewline
\hline 
 &  &  &  &  &  &  &  & \tabularnewline
1 & CC & ON & - &  &  &  & 0 & $(C/t)^{2}$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
2 & UC & OFF & + &  & - &  & $E_{a}$ & $e^{-E_{a}}(C/t)$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
3 & NC & ON & + &  & + &  & $\epsilon d$ & $(C/t)CS$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
4 & CU & OFF & + & - &  &  & $E_{a}$ & $e^{-E_{a}}(C/t)$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
5 & CN & ON & + & + &  &  & $\epsilon d$ & $(C/t)CS$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
6 & UU & OFF & + & - & - & - & $2E_{a}$ & $e^{-2E_{a}}$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
7 & UN & OFF & + & - & - & - & $E_{a}+\epsilon d$ & $e^{-E_{a}}CS$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
8 & NU & OFF & + & - & - & - & $E_{a}+\epsilon d$ & $e^{-E_{a}}CS$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
9 & $N_{x}N_{y}$ & ON & + & + & + & + & $\epsilon(d_{1}+d_{2})$ & $(CS)^{2}$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
10 & $N_{x}N_{x}$ & ON & + & + & + & + & $2\epsilon d$ & $(C/t)CS(2\epsilon,L)$\tabularnewline
 &  &  &  &  &  &  &  & \tabularnewline
\hline 
\end{tabular}

\caption{All possible binding configurations and the corresponding energies
for a combinatorial regulation setup implementing an AND gate. Each
gene has two binding sites which bind two different cognate TF types.
The ``configuration'' column lists all the configurations of the
two binding sites of a gene. 'C' denotes binding by cognate factor,
'N' - binding by noncognate and 'U' - means that the site is unbound.
We distinguish between binding of noncognate molecules of the same
type ($N_{x}N_{x}$) and different types ($N_{x}N_{y}$). The ``activity''
column denotes whether in the given configuration the gene is either
ON or OFF. To implement the AND gate, we assume that transcription
occurs (ON) only when both the binding sites are bound. The next four
columns denote whether this configuration is counted as crosstalk
(+) or not (-). In the leftmost column ``ON'', both the cognate
transcription factors are present (and the gene should be ON). In
the next three ``OFF'' columns, at least one of the cognate TFs
is absent (and the gene should be OFF). In ``C can be X'' column,
the cognate TF of only the left binding site (X) is present, in ``C
can be Y'', the cognate TF of only the right binding site is present,
and in ``C can be none'' column, both the cognate TFs are absent.
Blank space denotes a non-existing configuration: these are the configurations
including a cognate factor bound in the situation that it is absent.
The column ``Energy'' specifies the energy of these configurations.
We define the reference energetic level $E=0$ as the state 'CC' when
both sites are bound by their cognate factors, such that all other
energies are positive. The column ``Weight'' denotes the statistical
weight of the configurations, taking into account the concentrations
of the relevant TFs and the energy of the configurations. Note that
the statistical weight of the last binding configuration $N_{x}N_{x}$
uses $S(2\epsilon,L)$ instead of the otherwise $S(\epsilon,L)$.}


\end{table}

==> reverseComp.tex <==
\subsection{Optimal packing with reverse complement}
\label{sec:revComp}

We've also used an alternative definition of distance between sequences to compute the number of binding sites that one can pack in the optimal
packing setup. This definition of distance takes into
consideration the reverse complement as well of each sequence. If
$s_{i}$ and $s_{j}$ are two sequences with reverse complements $r_{i}$
and $r_{j}$ respectively, this new definition of Hamming distance
is

\begin{eqnarray}
HD_{rev}(s_{i},s_{j})=\min\Big[HD(s_{i},s_{j}),HD(r_{i},s_{j}),HD(s_{i},r_{j}),HD(r_{i},r_{j})\Big]
\end{eqnarray}

where $HD(s_i,s_j)$ is the usual Hamming distance as considered previously. This restricts the sequence space much more than with the usual definition
and as such, as seen in Fig. \ref{fig:bounds-rev}, we can pack fewer binding
sites in the sequence space at a specific $d_{\min}$. 

\begin{figure}[H]
\centering{\includegraphics[scale=0.7]{figures/rev_comp_L7}}

\caption{\textbf{Coding bounds for Hamming distance including reverse complement.} We
plot the number of binding site sequences that can be packed in the
sequence space for an optimal packing with different $d_{\min}$ at
$L=7$. The Singleton bound doesn't change from the usual situation
but the Gilbert-Varshamov bound, which takes into account the ``volume
of restricted ball'' around each sequence goes down. Because of stronger
constraints, the number of sequences that can be packed goes down
from the usual situation but only by a factor of $\approx2$. \label{fig:bounds-rev}}
\end{figure}
